Banach-valued modulation invariant Carleson embeddings and outer-$L^p$ spaces: the Walsh case

We prove modulation invariant embedding bounds from Bochner spaces $L^p(\mathbb{W};X)$ on the Walsh group to outer-$L^p$ spaces on the Walsh extended phase plane. The Banach space $X$ is assumed to be UMD and sufficiently close to a Hilbert space in an interpolative sense. Our embedding bounds imply $L^p$ bounds and sparse domination for the Banach-valued tritile operator, a discrete model of the Banach-valued bilinear Hilbert transform.

==> config/hyphenation.tex <==

\hyphenation{pro-duct de-fi-ning}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> config/layout.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

